Neural Randomized Planning for Whole Body Robot Motion

Robot motion planning has made vast advances over the past decades, but the challenge remains: robot mobile manipulators struggle to plan long-range whole-body motion in common household environments in real time, because of high-dimensional robot configuration space and complex environment geometry. To tackle the challenge, this paper proposes Neural Randomized Planner (NRP), which combines a global sampling-based motion planning (SBMP) algorithm and a local neural sampler. Intuitively, NRP uses the search structure inside the global planner to stitch together learned local sampling distributions to form a global sampling distribution adaptively. It benefits from both learning and planning. Locally, it tackles high dimensionality by learning to sample in promising regions from data, with a rich neural network representation. Globally, it composes the local sampling distributions through planning and exploits local geometric similarity to scale up to complex environments. Experiments both in simulation and on a real robot show \NRP yields superior performance compared to some of the best classical and learning-enhanced SBMP algorithms. Further, despite being trained in simulation, NRP demonstrates zero-shot transfer to a real robot operating in novel household environments, without any fine-tuning or manual adaptation.

==> macros.tex <==
%
% ACM style
%
\setlength{\textheight}{9.25in}
\setlength{\textwidth}{7in}
\setlength{\topmargin}{-0.25in}                     % 0.75in top margin
\addtolength{\topmargin}{-\headheight}
\addtolength{\topmargin}{-\headsep}
\setlength{\oddsidemargin}{-.25in}                  % 0.75in left margin
\setlength{\evensidemargin}{\oddsidemargin}
\setlength{\columnsep}{.33in}                       % gutter width

%
% IEEE style
%
\setlength{\textheight}{8.9in}
\setlength{\textwidth}{6.9in}
\setlength{\oddsidemargin}{-.16in}                  
\setlength{\evensidemargin}{\oddsidemargin}
\setlength{\columnsep}{.37in}                      % gutter width


%
% width for embedded text
%
\newlength{\minitextwidth}
\setlength{\minitextwidth}{\textwidth}
\addtolength{\minitextwidth}{-2.0cm}


%
% commands to reduce spacing between lines for 10pt documents
%
\newcommand{\tinylineskip}{\baselineskip=10pt}
\newcommand{\smalllineskip}{\baselineskip=11pt}
\newcommand{\normlineskip}{\baselineskip=12pt}


%
% customize caption fonts
%
\newcommand{\captionfonts}{\small}
\makeatletter                   % allow the use of @ in command names
\long\def\@makecaption#1#2{%
  \vskip\abovecaptionskip
  \sbox\@tempboxa{{\captionfonts #1. #2}}%
  \ifdim \wd\@tempboxa >\hsize
    {\captionfonts #1. #2\par}
  \else
    \hbox to\hsize{\hfil\box\@tempboxa\hfil}%
  \fi
  \vskip\belowcaptionskip}
\makeatother                    % cancel the effect of \makeatletter

%
% note format 
%
\def\note{
\pagestyle{empty}
\setlength{\oddsidemargin}{0pt}
\setlength{\evensidemargin}{0pt}
\setlength{\topmargin}{-0.3in}
\setlength{\headsep}{0pt}
\setlength{\textheight}{9in}
\setlength{\textwidth}{6.5in}

% heading information
% ##1 is flushed to the left, ##2 is flushed to the right
\def\notehead##1##2{\noindent {##1}\hfill {##2}\newline\medskip
     \rule[8pt]{\textwidth}{0.4pt}}
% title 
\def\notetitle##1{\medskip\centerline{\large \bf ##1}}
% section title
\def\noteitem##1{\subsection*{$\diamondsuit$ ##1}}
}


%
% theorems and proofs
%
\newtheorem{defn}{Definition}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{thm}[theorem]{Theorem}
\newtheorem{prop}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newenvironment{cor}{\noindent {\bf Corollary} \begin{it}}{ \end{it} }
\newcommand{\qed}{\mbox{}\hspace*{\fill}\nolinebreak\mbox{$\Box$}\smallskip}
\newenvironment{proof}{\par\noindent{\it Proof.}}{\(\qed\) \par}
\newenvironment{sketch}{\par\noindent{\it Proof Sketch.}}{\(\qed\) \par}

%
% asymptotic notation
%
\renewcommand{\O}[1]{\mbox{$O(#1)$}}
\newcommand{\Om}[1]{\mbox{$\Omega(#1)$}}
\newcommand{\Th}[1]{\mathit{\Theta(#1)}}

%
% vector notation
%
\newcommand{\del}{\nabla}                  % del operator
\newcommand{\dprod}{\cdot}                 % dot product and cross product
\newcommand{\cprod}{\times}
\newcommand{\vct}[1]{\mbox{{\bf #1}}}      % vector
\newcommand{\mat}[1]{\mbox{{\bf #1}}}      % matrix
\def\norm#1{\mbox{$\parallel#1\parallel$}}      % norm
\newcommand{\vnorm}[1]{\mbox{${            % vector norm
            \left|{\bf #1}\right|}$}}
\newcommand{\mnorm}[1]{                    % matrix norm
            \mbox{${\left\|{\bf #1}\right\|}$}}

%
% Greek letters
%
\newcommand{\veps}{\varepsilon}
\newcommand{\vpho}{\varpho}
\newcommand{\vphi}{\varphi}

%
% degree symbol
%
\newcommand{\degrees}[1]{\ensuremath{#1^\circ}}
% \DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\argmax}{\mathop{\mathrm{arg\,max}}}
\newcommand{\argmin}{\mathop{\mathrm{arg\,min}}}

%
% space symbol
%
\def\vs{{\tt \char'40}}






